Event fields: Capturing light fields at high speed, resolution, and dynamic range

Event cameras, which feature pixels that independently respond to changes in brightness, are becoming increasingly popular in high-speed applications due to their lower latency, reduced bandwidth requirements, and enhanced dynamic range compared to traditional frame-based cameras. Numerous imaging and vision techniques have leveraged event cameras for high-speed scene understanding by capturing high-framerate, high-dynamic range videos, primarily utilizing the temporal advantages inherent to event cameras. Additionally, imaging and vision techniques have utilized the light field-a complementary dimension to temporal information-for enhanced scene understanding. In this work, we propose "Event Fields", a new approach that utilizes innovative optical designs for event cameras to capture light fields at high speed. We develop the underlying mathematical framework for Event Fields and introduce two foundational frameworks to capture them practically: spatial multiplexing to capture temporal derivatives and temporal multiplexing to capture angular derivatives. To realize these, we design two complementary optical setups one using a kaleidoscope for spatial multiplexing and another using a galvanometer for temporal multiplexing. We evaluate the performance of both designs using a custom-built simulator and real hardware prototypes, showcasing their distinct benefits. Our event fields unlock the full advantages of typical light fields-like post-capture refocusing and depth estimation-now supercharged for high-speed and high-dynamic range scenes. This novel light-sensing paradigm opens doors to new applications in photography, robotics, and AR/VR, and presents fresh challenges in rendering and machine learning.

==> fig/table_template.tex <==



\begin{table}[ht]
    \setlength{\tabcolsep}{0em}
    \centering
    % \renewcommand*{\arraystretch}{0.75}
    \footnotesize
    \caption{
        Comparison of related work on thin cameras, where each criterion is fully~\greencheck, partially~\yellowcheck, or not~\redcheck met.
        See text for discussion.
        }
    \begin{tabularx}{\linewidth}{m{0.24\linewidth}XXXXXX}
    \toprule
    &
    {\footnotesize FlatCam \shortcite{asif2016flatcam}} &
    {\footnotesize DiffuserCam \shortcite{kuo2017diffusercam}} &
    {\footnotesize PiCam \shortcite{venkataraman2013picam}} &
    {\footnotesize Peng et al.~\shortcite{Peng2016DiffractiveAchromat}} &
    {\footnotesize Tseng et al.~\shortcite{neural_nanooptics}} &
    {\footnotesize Ours} \\
    \midrule
    \multicolumn{6}{l}{\textbf{Camera Characteristics}}\\ 
    \midrule
    On-Sensor (< 2mm) & 
    \green & 
    \yellow & 
    \green & 
    \red & 
    \green &
    \green \\
    Light Efficient & 
    \red & 
    \yellow & 
    \yellow & 
    \green & 
    \red &
    \green \\
    Broadband & 
    \green & 
    \green & 
    \green & 
    \yellow & 
    \yellow &
    \green \\
    Wide Field of View & 
    \yellow & 
    \yellow & 
    \yellow & 
    \red & 
    \yellow &
    \green \\
    MTF & 
    \red & 
    \red & 
    \yellow &
    \green & 
    \red  &
    \green \\
    Fabrication & 
    \green & 
    \yellow & 
    \red & 
    \red & 
    \green & 
    \green \\
    Well-posedness & 
    \red & 
    \red & 
    \yellow &
    \yellow & 
    \yellow  &
    \green \\
    \bottomrule
\end{tabularx}
    \label{tab:related_work}
\end{table}

==> sec/8_acknowledgment.tex <==
\section{Acknowledgment}
This project is funded by NSF grant 2403122.

We thank Laurence Rubin at Boston Craft Works, Joseph Poissant at Dartmouth Machine Shop, and Hannah Machesky at Two Way Mirrors for providing mirrors and polishing expertise for our kaleidoscope design.

We also extend our gratitude to the RISC lab members—Atul Agarwal, Dhawal Sirikonda, Kedari Chowtoori, and Sarah Friday—for their generous assistance in capturing the data. 

